Understanding Gamma-ray Burst Jet Structures from Afterglow Light Curves

Gamma-ray bursts (GRBs), associated with the collapse of massive stars or the collisions of compact objects, are the most luminous events in our universe. However, there is still much to learn about the nature of the relativistic jets launched from the central engines of these objects. We examine how jet structure - that is, the energy and velocity distribution as a function of angle - affects observed GRB afterglow light curves. Using the package afterglowpy, we compute light curves arising from an array of possible jet structures, and present the suite of models that can fit the coincident electromagnetic observations of GW190814 (which is likely due to a background AGN). Our work emphasizes not only the need for broadband spectral and timing data to distinguish among jet structure models, but also the necessity for high resolution radio follow-up to help resolve background sources that may mimic a GRB afterglow.

==> Makefile <==
LATEXMK=latexmk

SRC=header.tex \
    main.bib 

default: bhns

all: bhns

bhns: main.pdf

%.pdf: %.tex ${SRC} $(shell find figures/)
	${LATEXMK} -f -pdf $<

clean:
	rm -f ./*.aux ./*.bbl ./*.blg ./*.log ./*.nav ./*.out ./*.snm ./*.toc ./*.fls ./*.fdb_latexmk mainNotes.bib main.pdf


